Initialization for Nonnegative Matrix Factorization: a Comprehensive Review

Non-negative matrix factorization (NMF) has become a popular method for representing meaningful data by extracting a non-negative basis feature from an observed non-negative data matrix. Some of the unique features of this method in identifying hidden data put this method amongst the powerful methods in the machine learning area. The NMF is a known non-convex optimization problem and the initial point has a significant effect on finding an efficient local solution. In this paper, we investigate the most popular initialization procedures proposed for NMF so far. We describe each method and present some of their advantages and disadvantages. Finally, some numerical results to illustrate the performance of each algorithm are presented.

==> references.tex <==
@article{Elden,
  title={Numerical linear algebra and applications in data mining and IT},
  author={Eld{\'e}n, Lars},
  year={2003},
  publisher={Link{\"o}pings universitet}
}

@book{Skillicorn,
  title={Understanding complex datasets: data mining with matrix decompositions},
  author={Skillicorn, David},
  year={2007},
  publisher={Chapman and Hall/CRC}
}

@article{Friedland,
  title={Fast low rank approximations of matrices and tensors},
  author={Friedland, Shmuel and Mehrmann, V and Miedlar, A and Nkengla, M},
  journal={The Electronic Journal of Linear Algebra},
  volume={22},
  pages={1031--1048},
  year={2011}
}

@article{Kim,
  title={Matrix approximation under local low-rank assumption},
  author={Lee, Joonseok and Kim, Seungyeon and Lebanon, Guy and Singer, Yoram},
  journal={arXiv preprint arXiv:1301.3192},
  year={2013}
}

@book{Murphy,
  title={Machine learning: a probabilistic perspective},
  author={Murphy, Kevin P},
  year={2012},
  publisher={MIT press}
}
@article{Daniel,
  title={Learning the parts of objects by non-negative matrix factorization},
  author={Lee, Daniel D and Seung, H Sebastian},
  journal={Nature},
  volume={401},
  number={6755},
  pages={788--791},
  year={1999},
  publisher={Nature Publishing Group}
}
@misc{Amy2,
  title={Alternating least squares algorithms for the nonnegative matrix factorization},
  author={Langville, Amy N and Meyer, Carl D and Albright, Russell and Cox, James and Duling, David},
  year={2006},
  publisher={Unpublished}
}



@article{Lee01,
  title={Algorithms for Non-Negative Matrix Factorization. NIPS (2000)},
  author={Lee, DD and Seung, HS},
  journal={Google Scholar},
  pages={556--562}
}
@article{Aggarwal,
  title={Data clustering},
  author={Aggarwal, Charu C and Reddy, Chandan K},
  journal={Algorithms and applications. Chapman\&Hall/CRC Data mining and Knowledge Discovery series, Londra},
  year={2014},
  publisher={Citeseer}
}

@article{Zheng,
  title={Initialization enhancer for non-negative matrix factorization},
  author={Zheng, Zhonglong and Yang, Jie and Zhu, Yitan},
  journal={Engineering Applications of Artificial Intelligence},
  volume={20},
  number={1},
  pages={101--110},
  year={2007},
  publisher={Elsevier}
}

@article{Mahoney,
  title={Randomized algorithms for matrices and data},
  author={Mahoney, Michael W},
  journal={arXiv preprint arXiv:1104.5557},
  year={2011}
}

@article{Drineas,
  title={RandNLA: randomized numerical linear algebra},
  author={Drineas, Petros and Mahoney, Michael W},
  journal={Communications of the ACM},
  volume={59},
  number={6},
  pages={80--90},
  year={2016},
  publisher={ACM New York, NY, USA}
}

@inproceedings{Wangli,
  title={Efficient nonnegative matrix factorization with random projections},
  author={Wang, Fei and Li, Ping},
  booktitle={Proceedings of the 2010 SIAM International Conference on Data Mining},
  pages={281--292},
  year={2010},
  organization={SIAM}
}

@article{Tepper,
  title={Compressed nonnegative matrix factorization is fast and accurate},
  author={Tepper, Mariano and Sapiro, Guillermo},
  journal={IEEE Transactions on Signal Processing},
  volume={64},
  number={9},
  pages={2269--2283},
  year={2016},
  publisher={IEEE}
}

@inproceedings{Zhou,
  title={Bilateral random projections},
  author={Zhou, Tianyi and Tao, Dacheng},
  booktitle={2012 IEEE International Symposium on Information Theory Proceedings},
  pages={1286--1290},
  year={2012},
  organization={IEEE}
}

@techreport{Albright,
  title={Algorithms, initializations, and convergence for the nonnegative matrix factorization},
  author={Albright, Russell and Cox, James and Duling, David and Langville, Amy N and Meyer, C},
  year={2006},
  institution={Tech. rep. 919. NCSU Technical Report Math 81706. http://meyer. math. ncsu~…}
}

@book{Berthold,
  title={Guide to intelligent data analysis: how to intelligently make sense of real data},
  author={Berthold, Michael R and Borgelt, Christian and H{\"o}ppner, Frank and Klawonn, Frank},
  year={2010},
  publisher={Springer Science \& Business Media}
}

@inproceedings{xu,
  title={Document clustering based on non-negative matrix factorization},
  author={Xu, Wei and Liu, Xin and Gong, Yihong},
  booktitle={Proceedings of the 26th annual international ACM SIGIR conference on Research and development in informaion retrieval},
  pages={267--273},
  year={2003}
}

@article{Chretien,
  title={A Bregman-proximal point algorithm for robust non-negative matrix factorization with possible missing values and outliers-application to gene expression analysis},
  author={Chr{\'e}tien, St{\'e}phane and Guyeux, Christophe and Conesa, Bastien and Delage-Mouroux, R{\'e}gis and Jouvenot, Mich{\`e}le and Huetz, Philippe and Desc{\^o}tes, Fran{\c{c}}oise},
  journal={BMC bioinformatics},
  volume={17},
  number={8},
  pages={623--631},
  year={2016},
  publisher={Springer}
}

@book{Cichocki4,
  title={Adaptive blind signal and image processing: learning algorithms and applications},
  author={Cichocki, Andrzej and Amari, Shun-ichi},
  year={2002},
  publisher={John Wiley \& Sons}
}

@misc{Shahnaz,
  title={Clustering using non-negative matrix factorization on sparse graphs},
  author={Perronnin, Florent and Bouchard, Guillaume},
  year={2017},
  month=aug # "~8",
  publisher={Google Patents},
  note={US Patent 9,727,532}
}
@article{Wild04,
  title={Improving non-negative matrix factorizations through structured initialization},
  author={Wild, Stefan and Curry, James and Dougherty, Anne},
  journal={Pattern recognition},
  volume={37},
  number={11},
  pages={2217--2232},
  year={2004},
  publisher={Elsevier}
}
@phdthesis{Wild02,
  title={Seeding non-negative matrix factorizations with the spherical k-means clustering},
  author={Wild, Stefan and Wild, Written Stefan and Curry, James and Dougherty, Anne and Betterton, Meredith},
  year={2003},
  school={Citeseer}
}


@article{Forgy,
  title={Cluster analysis of multivariate data: Efficiency vs. interpretability of classification},
  author={Forgey, Edward},
  journal={Biometrics},
  volume={21},
  number={3},
  pages={768--769},
  year={1965},
  publisher={Oxford}
}
@book{Hartigan,
  title={Clustering algorithms},
  author={Hartigan, John A},
  year={1975},
  publisher={John Wiley \& Sons, Inc.}
}
@inproceedings{Ding},
  title={On the equivalence of nonnegative matrix factorization and spectral clustering},
  author={Ding, Chris and He, Xiaofeng and Simon, Horst D},
  booktitle={Proceedings of the 2005 SIAM international conference on data mining},
  pages={606--610},
  year={2005},
  organization={SIAM}
}
@book{Anderberg,
  title={Cluster analysis for applications: probability and mathematical statistics: a series of monographs and textbooks},
  author={Anderberg, Michael R},
  volume={19},
  year={2014},
  publisher={Academic press}
}

@article{Xue08,
  title={Clustering-based initialization for non-negative matrix factorization},
  author={Xue, Yun and Tong, Chong Sze and Chen, Ying and Chen, Wen-Sheng},
  journal={Applied Mathematics and Computation},
  volume={205},
  number={2},
  pages={525--536},
  year={2008},
  publisher={Elsevier}
}
@article{Dong,
  title={Nonnegative rank factorization—a heuristic approach via rank reduction},
  author={Dong, Bo and Lin, Matthew M and Chu, Moody T},
  journal={Numerical Algorithms},
  volume={65},
  number={2},
  pages={251--274},
  year={2014},
  publisher={Springer}
}

@article{Goldberg,
  title={Genetic algorithms and machine learning},
  author={Goldberg, David E and Holland, John Henry},
  year={1988},
  publisher={Kluwer Academic Publishers-Plenum Publishers; Kluwer Academic Publishers~…}
}

@inproceedings{Stadlthanner,
  title={Sparse nonnegative matrix factorization with genetic algorithms for microarray analysis},
  author={Stadlthanner, Kurt and Lutter, Dominik and Theis, Fabian J and Lang, Elmar Wolfgang and Tom{\'e}, Ana Maria and Georgieva, Petia and Puntonet, Carlos Garc{\'\i}a},
  booktitle={2007 International Joint Conference on Neural Networks},
  pages={294--299},
  year={2007},
  organization={IEEE}
}



@article{asel,
  title={Developing genetic algorithms for boolean matrix factorization},
  author={Sn{\'a}{\v{s}}el, V{\'a}clav and Plato{\v{s}}, Jan and Kr{\"o}mer, Pavel},
  journal={Databases, Texts},
  volume={61},
  year={2008}
}

@inproceedings{Kennedy,
  title={Particle swarm optimization},
  author={Eberhart, Russell and Kennedy, James},
  booktitle={Proceedings of the IEEE international conference on neural networks},
  volume={4},
  pages={1942--1948},
  year={1995},
  organization={Citeseer}
}


@book{Price,
  title={Differential evolution: a practical approach to global optimization},
  author={Price, Kenneth and Storn, Rainer M and Lampinen, Jouni A},
  year={2006},
  publisher={Springer Science \& Business Media}
}

@article{Boutsidis,
  title={SVD based initialization: A head start for nonnegative matrix factorization},
  author={Boutsidis, Christos and Gallopoulos, Efstratios},
  journal={Pattern recognition},
  volume={41},
  number={4},
  pages={1350--1362},
  year={2008},
  publisher={Elsevier}
}

@article{S.Deerwester,
  title={Indexing by latent semantic analysis},
  author={Deerwester, Scott and Dumais, Susan T and Furnas, George W and Landauer, Thomas K and Harshman, Richard},
  journal={Journal of the American society for information science},
  volume={41},
  number={6},
  pages={391--407},
  year={1990},
  publisher={Wiley Online Library}
}

@article{Eckart,
  title={The approximation of one matrix by another of lower rank},
  author={Eckart, Carl and Young, Gale},
  journal={Psychometrika},
  volume={1},
  number={3},
  pages={211--218},
  year={1936},
  publisher={Springer}
}
@article{Lijie,
  title={Singular value decomposition applied to digital image processing},
  author={Cao, Lijie},
  journal={Division of Computing Studies, Arizona State University Polytechnic Campus, Mesa, Arizona State University polytechnic Campus},
  pages={1--15},
  year={2006}
}

@article{g1,
  title={A scaled gradient projection method for constrained image deblurring},
  author={Bonettini, Silvia and Zanella, Riccardo and Zanni, Luca},
  journal={Inverse problems},
  volume={25},
  number={1},
  pages={015002},
  year={2008},
  publisher={IOP Publishing}
}
@article{g2,
  title={NeNMF: An optimal gradient method for nonnegative matrix factorization},
  author={Guan, Naiyang and Tao, Dacheng and Luo, Zhigang and Yuan, Bo},
  journal={IEEE Transactions on Signal Processing},
  volume={60},
  number={6},
  pages={2882--2898},
  year={2012},
  publisher={IEEE}
}
@article{g3,
  title={Efficient nonnegative matrix factorization via projected Newton method},
  author={Gong, Pinghua and Zhang, Changshui},
  journal={Pattern Recognition},
  volume={45},
  number={9},
  pages={3557--3565},
  year={2012},
  publisher={Elsevier}
}
@article{g4,
  title={Quadratic regularization projected Barzilai--Borwein method for nonnegative matrix factorization},
  author={Huang, Yakui and Liu, Hongwei and Zhou, Shuisheng},
  journal={Data mining and knowledge discovery},
  volume={29},
  number={6},
  pages={1665--1684},
  year={2015},
  publisher={Springer}
}
@article{g5,
  title={An interior-point algorithm for linearly constrained convex optimization based on kernel function and application in non-negative matrix factorization},
  author={Fathi-Hafshejani, S and Moaberfard, Z},
  journal={Optimization and Engineering},
  volume={21},
  number={3},
  pages={1019--1051},
  year={2020},
  publisher={Springer}
}
@article{Qiao,
  title={New SVD based initialization strategy for non-negative matrix factorization},
  author={Qiao, Hanli},
  journal={Pattern Recognition Letters},
  volume={63},
  pages={71--77},
  year={2015},
  publisher={Elsevier}
}
@inproceedings{Amy3,
  title={Initializations for the nonnegative matrix factorization},
  author={Langville, Amy N and Meyer, Carl D and Albright, Russell and Cox, James and Duling, David},
  booktitle={Proceedings of the twelfth ACM SIGKDD international conference on knowledge discovery and data mining},
  pages={23--26},
  year={2006},
  organization={Citeseer}
}
@book{Cichocki3,
  title={Nonnegative matrix and tensor factorizations: applications to exploratory multi-way data analysis and blind source separation},
  author={Cichocki, Andrzej and Zdunek, Rafal and Phan, Anh Huy and Amari, Shun-ichi},
  year={2009},
  publisher={John Wiley \& Sons}
}
@article{Guillamet,
  title={Evaluation of distance metrics for recognition based on non-negative matrix factorization},
  author={Guillamet, David and Vitria, Jordi},
  journal={Pattern Recognition Letters},
  volume={24},
  number={9-10},
  pages={1599--1605},
  year={2003},
  publisher={Elsevier}
}

@article{Turk,
  title={Eigenfaces for recognition},
  author={Turk, Matthew and Pentland, Alex},
  journal={Journal of cognitive neuroscience},
  volume={3},
  number={1},
  pages={71--86},
  year={1991},
  publisher={MIT Press One Rogers Street, Cambridge, MA 02142-1209, USA journals-info~…}
}
@article{Shen,
  title={Sparse principal component analysis via regularized low rank matrix approximation},
  author={Shen, Haipeng and Huang, Jianhua Z},
  journal={Journal of multivariate analysis},
  volume={99},
  number={6},
  pages={1015--1034},
  year={2008},
  publisher={Elsevier}
}
@inproceedings{Zass,
  title={Nonnegative sparse PCA},
  author={Zass, Ron and Shashua, Amnon},
  booktitle={Advances in neural information processing systems},
  pages={1561--1568},
  year={2007},
  organization={Citeseer}
}

@article{Snasel,
  title={Developing genetic algorithms for boolean matrix factorization},
  author={Sn{\'a}{\v{s}}el, V{\'a}clav and Plato{\v{s}}, Jan and Kr{\"o}mer, Pavel},
  journal={Databases, Texts},
  volume={61},
  year={2008}
}


@inproceedings{sandler,
  title={On the use of linear programming for unsupervised text classification},
  author={Sandler, Mark},
  booktitle={Proceedings of the eleventh ACM SIGKDD international conference on Knowledge discovery in data mining},
  pages={256--264},
  year={2005}
}

@inproceedings{Zhao08,
  title={Facial expression recognition based on PCA and NMF},
  author={Zhao, Lihong and Zhuang, Guibin and Xu, Xinhe},
  booktitle={2008 7th World Congress on Intelligent Control and Automation},
  pages={6826--6829},
  year={2008},
  organization={IEEE}
}
@article{Xiu-rui-16,
  title={Non-negative matrix factorization based unmixing for principal component transformed hyperspectral data},
  author={Geng, Xiu-rui and Ji, Lu-yan and Sun, Kang},
  journal={Frontiers of Information Technology \& Electronic Engineering},
  volume={17},
  number={5},
  pages={403--412},
  year={2016},
  publisher={Springer}
}
@inproceedings{Benachir,
  title={Modified independent component analysis for initializing non-negative matrix factorization: An approach to hyperspectral image unmixing},
  author={Benachir, Djaouad and Hosseini, Shahram and Deville, Yannick and Karoui, Moussa Sofiane and Hameurlain, Abdelkader},
  booktitle={2013 IEEE 11th International Workshop of Electronics, Control, Measurement, Signals and their application to Mechatronics},
  pages={1--6},
  year={2013},
  organization={IEEE}
}
@article{Oja,
  title={Blind separation of positive sources by globally convergent gradient search},
  author={Oja, Erkki and Plumbley, Mark},
  journal={Neural Computation},
  volume={16},
  number={9},
  pages={1811--1825},
  year={2004},
  publisher={MIT Press One Rogers Street, Cambridge, MA 02142-1209, USA journals-info~…}
}
@inproceedings{Kitamura,
  title={Efficient initialization for nonnegative matrix factorization based on nonnegative independent component analysis},
  author={Kitamura, Daichi and Ono, Nobutaka},
  booktitle={2016 IEEE International Workshop on Acoustic Signal Enhancement (IWAENC)},
  pages={1--5},
  year={2016},
  organization={IEEE}
}
@article{37,
  title={When does non-negative matrix factorization give a correct decomposition into parts?},
  author={Donoho, David L and Stodden, Victoria C},
  year={2004}
}
@article{8,
  title={Singular value decomposition for genome-wide expression data processing and modeling},
  author={Alter, Orly and Brown, Patrick O and Botstein, David},
  journal={Proceedings of the National Academy of Sciences},
  volume={97},
  number={18},
  pages={10101--10106},
  year={2000},
  publisher={National Acad Sciences}
}
@incollection{17,
  title={Singular value decomposition and principal component analysis},
  author={Wall, Michael E and Rechtsteiner, Andreas and Rocha, Luis M},
  booktitle={A practical approach to microarray data analysis},
  pages={91--109},
  year={2003},
  publisher={Springer}
}
@article{14,
  title={Dimension reduction techniques for the integrative analysis of multi-omics data},
  author={Meng, Chen and Zeleznik, Oana A and Thallinger, Gerhard G and Kuster, Bernhard and Gholami, Amin M and Culhane, Aed{\'\i}n C},
  journal={Briefings in bioinformatics},
  volume={17},
  number={4},
  pages={628--641},
  year={2016},
  publisher={Oxford University Press}
}
@article{3,
  title={Enter the matrix: factorization uncovers knowledge from omics},
  author={Stein-O’Brien, Genevieve L and Arora, Raman and Culhane, Aedin C and Favorov, Alexander V and Garmire, Lana X and Greene, Casey S and Goff, Loyal A and Li, Yifeng and Ngom, Aloune and Ochs, Michael F and others},
  journal={Trends in Genetics},
  volume={34},
  number={10},
  pages={790--805},
  year={2018},
  publisher={Elsevier}
}
@article{19,
  title={A non-negative matrix factorization method for detecting modules in heterogeneous omics multi-modal data},
  author={Yang, Zi and Michailidis, George},
  journal={Bioinformatics},
  volume={32},
  number={1},
  pages={1--8},
  year={2016},
  publisher={Oxford University Press}
}
@article{20,
  title={Improving knowledge on the activation of bone marrow fibroblasts in MGUS and MM disease through the automatic extraction of genes via a nonnegative matrix factorization approach on gene expression profiles},
  author={Boccarelli, Angelina and Esposito, Flavia and Coluccia, Mauro and Frassanito, Maria Antonia and Vacca, Angelo and Del Buono, Nicoletta},
  journal={Journal of translational medicine},
  volume={16},
  number={1},
  pages={1--16},
  year={2018},
  publisher={Springer}
}
@article{21,
  title={Multi-omic and multi-view clustering algorithms: review and cancer benchmark},
  author={Rappoport, Nimrod and Shamir, Ron},
  journal={Nucleic acids research},
  volume={46},
  number={20},
  pages={10546--10562},
  year={2018},
  publisher={Oxford University Press}
}
@article{22,
  title={Orthogonal joint sparse NMF for microarray data analysis},
  author={Esposito, Flavia and Gillis, Nicolas and Del Buono, Nicoletta},
  journal={Journal of mathematical biology},
  volume={79},
  number={1},
  pages={223--247},
  year={2019},
  publisher={Springer}
}
@article{23,
  title={Nonnegative Matrix Factorization models for knowledge extraction from biomedical and other real world data},
  author={Esposito, Flavia and Del Buono, Nicoletta and Selicato, Laura},
  journal={PAMM},
  volume={20},
  number={1},
  pages={e202000032},
  year={2021},
  publisher={Wiley Online Library}
}
@article{18,
  title={Independent component analysis for unraveling the complexity of cancer omics datasets},
  author={Sompairac, Nicolas and Nazarov, Petr V and Czerwinska, Urszula and Cantini, Laura and Biton, Anne and Molkenov, Askhat and Zhumadilov, Zhaxybay and Barillot, Emmanuel and Radvanyi, Francois and Gorban, Alexander and others},
  journal={International Journal of molecular sciences},
  volume={20},
  number={18},
  pages={4414},
  year={2019},
  publisher={Multidisciplinary Digital Publishing Institute}
}
@article{Golub,
  title={Matrix computations 3rd edition},
  author={Golub, Gene H and Van Loan, Charles F},
  journal={The John Hopkins University, Baltimore},
  year={1996}
}
@article{Tamara,
  title={A semidiscrete matrix decomposition for latent semantic indexing information retrieval},
  author={Kolda, Tamara G and O'leary, Dianne P},
  journal={ACM Transactions on Information Systems (TOIS)},
  volume={16},
  number={4},
  pages={322--346},
  year={1998},
  publisher={ACM New York, NY, USA}
}
@book{Datta,
  title={Numerical linear algebra and applications},
  author={Datta, Biswa Nath},
  volume={116},
  year={2010},
  publisher={Siam}
}
@article{Petros,
  title={Fast Monte Carlo algorithms for matrices III: Computing a compressed approximate matrix decomposition},
  author={Drineas, Petros and Kannan, Ravi and Mahoney, Michael W},
  journal={SIAM Journal on Computing},
  volume={36},
  number={1},
  pages={184--206},
  year={2006},
  publisher={SIAM}
}

@book{Smilde,
  title={Multi-way analysis: applications in the chemical sciences},
  author={Smilde, Age and Bro, Rasmus and Geladi, Paul},
  year={2005},
  publisher={John Wiley \& Sons}
}
@book{Sundarapandian,
  title={Numerical linear algebra},
  author={Sundarapandian, V},
  year={2008},
  publisher={PHI Learning Pvt. Ltd.}
}
@book{Meyer,
  title={Matrix analysis and applied linear algebra},
  author={Meyer, Carl D},
  volume={71},
  year={2000},
  publisher={Siam}
}
@book{Trefethen,
  title={Numerical linear algebra},
  author={Trefethen, Lloyd N and Bau III, David},
  volume={50},
  year={1997},
  publisher={Siam}
}
@article{Fazel,
  title={Guaranteed minimum-rank solutions of linear matrix equations via nuclear norm minimization},
  author={Recht, Benjamin and Fazel, Maryam and Parrilo, Pablo A},
  journal={SIAM review},
  volume={52},
  number={3},
  pages={471--501},
  year={2010},
  publisher={SIAM}
}

@misc{Reinsel,
  title={Multivariate Reduced Rank Regression, Theory and Applications},
  author={Paruolo, Paolo},
  year={2000},
  publisher={JSTOR}
}
@article{Miller,
  title={Identification of linear time-invariant systems via constrained step-based realization},
  author={Miller, Daniel N and de Callafon, Raymond A},
  journal={IFAC Proceedings Volumes},
  volume={45},
  number={16},
  pages={1155--1160},
  year={2012},
  publisher={Elsevier}
}
@article{Chu,
  title={Structured low rank approximation},
  author={Chu, Moody T and Funderlic, Robert E and Plemmons, Robert J},
  journal={Linear algebra and its applications},
  volume={366},
  pages={157--172},
  year={2003},
  publisher={Elsevier}
}
@article{Chan,
  title={Rank revealing QR factorizations},
  author={Chan, Tony F},
  journal={Linear algebra and its applications},
  volume={88},
  pages={67--82},
  year={1987},
  publisher={Elsevier}
}
@article{Golub68,
  title={Linear least squares solutions by Householder transformations},
  author={Businger, Peter and Golub, Gene H},
  journal={Numerische Mathematik},
  volume={7},
  number={3},
  pages={269--276},
  year={1965},
  publisher={Springer}
}
@techreport{Golub69,
  title={Rank degeneracy and least squares problems},
  author={Golub, Gene and Klema, Virginia and Stewart, Gilbert W},
  year={1976},
  institution={STANFORD UNIV CA DEPT OF COMPUTER SCIENCE}
}
@article{Gu,
  title={Efficient algorithms for computing a strong rank-revealing QR factorization},
  author={Gu, Ming and Eisenstat, Stanley C},
  journal={SIAM Journal on Scientific Computing},
  volume={17},
  number={4},
  pages={848--869},
  year={1996},
  publisher={SIAM}
}
@article{Zheng07,
  title={Initialization enhancer for non-negative matrix factorization},
  author={Zheng, Zhonglong and Yang, Jie and Zhu, Yitan},
  journal={Engineering Applications of Artificial Intelligence},
  volume={20},
  number={1},
  pages={101--110},
  year={2007},
  publisher={Elsevier}

}
@article{Casalino,
  title={Subtractive clustering for seeding non-negative matrix factorizations},
  author={Casalino, Gabriella and Del Buono, Nicoletta and Mencar, Corrado},
  journal={Information Sciences},
  volume={257},
  pages={369--387},
  year={2014},
  publisher={Elsevier}
}
@article{Rezaei,
  title={An efficient initialization method for nonnegative matrix factorization},
  author={Rezaei, M and Boostani, R and Rezaei, M},
  journal={Journal of Applied Sciences},
  volume={11},
  number={2},
  pages={354--359},
  year={2011}
}
@inproceedings{Alshabrawy,
  title={Underdetermined blind source separation based on fuzzy c-means and semi-nonnegative matrix factorization},
  author={Alshabrawy, Ossama S and Ghoneim, ME and Awad, WA and Hassanien, Aboul Ella},
  booktitle={2012 Federated Conference on Computer Science and Information Systems (FedCSIS)},
  pages={695--700},
  year={2012},
  organization={IEEE}
}
@inproceedings{kim07,
  title={A method of initialization for nonnegative matrix factorization},
  author={Kim, Yong-Deok and Choi, Seungjin},
  booktitle={2007 IEEE International Conference on Acoustics, Speech and Signal Processing-ICASSP'07},
  volume={2},
  pages={II--537},
  year={2007},
  organization={IEEE}
}
@inproceedings{Janecek,
  title={Using population based algorithms for initializing nonnegative matrix factorization},
  author={Janecek, Andreas and Tan, Ying},
  booktitle={International Conference in Swarm Intelligence},
  pages={307--316},
  year={2011},
  organization={Springer}
}
@article{syed,
  title={Improved SVD-based initialization for nonnegative matrix factorization using low-rank correction},
  author={Atif, Syed Muhammad and Qazi, Sameer and Gillis, Nicolas},
  journal={Pattern Recognition Letters},
  volume={122},
  pages={53--59},
  year={2019},
  publisher={Elsevier}
}
@inproceedings{pro1,
  title={Rank-one NMF-based initialization for NMF and relative error bounds under a geometric assumption},
  author={Liu, Zhaoqiang and Tan, Vincent YF},
  booktitle={2018 Information Theory and Applications Workshop (ITA)},
  pages={1--15},
  year={2018},
  organization={IEEE}
}
@inproceedings{pro2,
  title={Initialization of nonnegative matrix factorization with vertices of convex polytope},
  author={Zdunek, Rafal},
  booktitle={International Conference on Artificial Intelligence and Soft Computing},
  pages={448--455},
  year={2012},
  organization={Springer}
}
@article{pro3,
  title={The successive projection algorithm as an initialization method for brain tumor segmentation using non-negative matrix factorization},
  author={Sauwen, Nicolas and Acou, Marjan and Bharath, Halandur N and Sima, Diana M and Veraart, Jelle and Maes, Frederik and Himmelreich, Uwe and Achten, Eric and Van Huffel, Sabine},
  journal={Plos one},
  volume={12},
  number={8},
  pages={e0180268},
  year={2017},
  publisher={Public Library of Science San Francisco, CA USA}
}
@inproceedings{29,
  title={A Purely Geometric Approach to Non-Negative Matrix Factorization.},
  author={Bauckhage, Christian},
  booktitle={LWA},
  pages={125--136},
  year={2014},
  organization={Citeseer}
}
@article{30,
  title={A probabilistic latent variable model for acoustic modeling},
  author={Smaragdis, Paris and Raj, Bhiksha and Shashanka, Madhusudana},
  journal={Advances in models for acoustic processing, NIPS},
  volume={148},
  pages={8--1},
  year={2006},
  publisher={Citeseer}
}
@article{math,
  title={A Review on Initialization Methods for Nonnegative Matrix Factorization: Towards Omics Data Experiments},
  author={Esposito, Flavia},
  journal={Mathematics},
  volume={9},
  number={9},
  pages={1006},
  year={2021},
  publisher={Multidisciplinary Digital Publishing Institute}
}
